Deep Underground Neutrino Experiment (DUNE), Far Detector Technical Design Report, Volume III: DUNE Far Detector Technical Coordination

The preponderance of matter over antimatter in the early universe, the dynamics of the supernovae that produced the heavy elements necessary for life, and whether protons eventually decay -- these mysteries at the forefront of particle physics and astrophysics are key to understanding the early evolution of our universe, its current state, and its eventual fate. The Deep Underground Neutrino Experiment (DUNE) is an international world-class experiment dedicated to addressing these questions as it searches for leptonic charge-parity symmetry violation, stands ready to capture supernova neutrino bursts, and seeks to observe nucleon decay as a signature of a grand unified theory underlying the standard model. The DUNE far detector technical design report (TDR) describes the DUNE physics program and the technical designs of the single- and dual-phase DUNE liquid argon TPC far detector modules. Volume III of this TDR describes how the activities required to design, construct, fabricate, install, and commission the DUNE far detector modules are organized and managed. This volume details the organizational structures that will carry out and/or oversee the planned far detector activities safely, successfully, on time, and on budget. It presents overviews of the facilities, supporting infrastructure, and detectors for context, and it outlines the project-related functions and methodologies used by the DUNE technical coordination organization, focusing on the areas of integration engineering, technical reviews, quality assurance and control, and safety oversight. Because of its more advanced stage of development, functional examples presented in this volume focus primarily on the single-phase (SP) detector module.

==> generated/req-DP-INST-01.tex <==
   
  \newtag{DP-INST-1}{ spec:handling-specs }  & Compliance with the material handling specification for all material transported underground  &  Fulfill material handling specification &  Being able to tranport undergound the equipment &  Material documentation and inspection \\ \colhline
    

==> generated/req-DP-INST-02.tex <==
   
  \newtag{DP-INST-2}{ spec:material-buffer }  & Material buffer at the warehouse facility  &  >1 month &  Limit the impact of delivery delays on the installation schedule &  Regular report from the construction sites \\ \colhline
    

==> generated/req-DP-INST-03.tex <==
   
  \newtag{DP-INST-3}{ spec:underground-storage }  & Material storage available underground  &  >4~\dshorts{crp} &  Limit the impact of rejected detector components on the installation schedule &  Dedicated space to store the detector component available undergorund in the vicinity of the clean room \\ \colhline
    

==> generated/req-DP-INST-04.tex <==
   
  \newtag{DP-INST-4}{ spec:clean-room-specs }  & Cryostat and clean room environment  &  >ISO-8 &  Safe handling of the detector components and limit the radioactive background &  Regular air quality checks, constant air filtering, regular cleaning of the clean room and the cryostat, use of clean room equipment \\ \colhline
    

==> generated/req-DP-INST-05.tex <==
   
  \newtag{DP-INST-5}{ spec:cold-box-cryo }  & Cold box cryogenics system  &  Independent operation of the four cold boxes &  Guarantee the needed flexibility in the tests &  Simultaneous operation of the cold boxes \\ \colhline
    

==> generated/req-longtable-DP-INST.tex <==
% This file is generated, any edits may be lost.
\begin{footnotesize}
%\begin{longtable}{p{0.14\textwidth}p{0.13\textwidth}p{0.18\textwidth}p{0.22\textwidth}p{0.20\textwidth}}
\begin{longtable}{p{0.12\textwidth}p{0.18\textwidth}p{0.17\textwidth}p{0.25\textwidth}p{0.16\textwidth}}
\caption{DP installation specifications  \fixmehl{ref \texttt{tab:spec:DP-INST}}} \\
  \rowcolor{dunesky}
       Label & Description  & Specification \newline (Goal) & Rationale & Validation \\  \colhline


\input{generated/req-DP-INST-01.tex}
\input{generated/req-DP-INST-02.tex}
\input{generated/req-DP-INST-03.tex}
\input{generated/req-DP-INST-04.tex}
\input{generated/req-DP-INST-05.tex}


\label{tab:specs:DP-INST}
\end{longtable}
\end{footnotesize}

==> generated/reqdefs-DP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CALIB


\def\dpdatavolumelaser{$>\,\SI{37}{TB/yr/10 kt}$}
\def\dpdatavolumepns{$>\,\SI{170}{TB/yr/10 kt}$}
\def\dpefieldcalibcoverage{$>\,\SI{93}{\%}$}
\def\dpefieldcalibgranularity{\SI{10 x 10 x 10}{\centi\metre}}
\def\dpefieldcalibprecision{\SI{1}{\%}}
\def\dplaserpositionprecision{\SI{0.5}{\milli\radian}}
\def\dpneutronsourcecoverage{$>\,\SI{75}{\%}$}


==> generated/reqdefs-DP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CISC


\def\dpcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\dpeleclifetimeprec{$<\,$2.3\%}
\def\dpeleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\dpinstefield{$<\,\SI{30}{kV/cm}$}
\def\dpinstnoise{$<<\,\SI{1000}\,e^- $}
\def\dpslowcontrolalarmrate{$<\,$150/day}
\def\dpslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\dpslowcontrolnumvars{$>\,\num{150000}$}
\def\dptemprepro{$<\,\SI{5}{mK}$}
\def\dptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-DP-CRP.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CRP


\def\dpcrpvertprecision{$<\,\SI{1}{\milli\meter}$}


==> generated/reqdefs-DP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-DAQ


\def\dpdaqdeadtime{}
\def\dpDAQreadout{\SI{65}{GB/s} per dual phase detector module}
\def\dpDAQreadoutwindow{\SI{10}{\micro\second} < readout window < \SI{100}{s}}
\def\dpDAQthroughput{\SI{2}{GB/s} average storage throughput; \SI{100}{GB/s} peak temporary storage throughput per dual phase detector module}
\def\dpdatarecord{}
\def\dpdataverification{}
\def\dptriggercalibration{}
\def\dptriggerhighenergy{$>\,$\SI{100}{\MeV}}
\def\dptriggerlowenergy{$>\,$\SI{10}{\MeV}}


==> generated/reqdefs-DP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-ELEC




==> generated/reqdefs-DP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-FD


\def\dp{}
\def\dpdenonfenoise{$<<\,\SI{1000}\,e^- $}
\def\dpdpadcnumberofbits{\num{12} bits}
\def\dpdpadcsamplingfreq{$\sim\,\SI{2.5}{\mega\hertz}$}
\def\dpdpcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\dpdpcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\dpdpcrpeffgain{\num{6}}
\def\dpdpcrpgaps{$<\,\SI{30}{mm}$ between adjacent CRPs}
\def\dpdpcrpplanarity{$\pm\,\SI{0.5}{mm}$}
\def\dpdpcrpstripspacing{$<\,\SI{4.7}{mm}$}
\def\dpdpcryomonitordevices{}
\def\dpdpdataratetotape{$<\,\SI{30}{PB/year}$}
\def\dpdpdeadchannels{$<\,\SI{1}{\%}$}
\def\dpdpdetmoduptime{$>\,$90\%}
\def\dpdpdetuptime{$>\,$98\%}
\def\dpdpfepeaktime{\SI{1}{\micro\second}}
\def\dpdphvpsripple{$<\,\SI{100}e^-$}
\def\dpdphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\dpdplarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\dpdplarncontamination{$<\,\SI{3}{ppm}$}
\def\dpdplarpurity{$>$\,\SI{5}{ms}}
\def\dpdplightyield{$>\,\SI{1}{PE/MeV}$ (at anode), $>\,\SI{5}{PE/MeV}$ (avg  over active volume)}
\def\dpdplocalefields{$<\,\SI{30}{kV/cm}$}
\def\dpdpmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\dpdpmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\dpdpradiopurity{less than that from $^{39}$Ar}
\def\dpdpsignalsaturation{\num{7500000} electrons}
\def\dpdpsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\dpdpsystemnoise{$<\,\SI{1000}\,e^-$}
\def\dpdptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-DP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-HV


\def\dphvdbredundancy{$>\,\num{2}$ HVDB chain}


==> generated/reqdefs-DP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-INST


\def\dpcleanroomspecs{>ISO-8}
\def\dpcoldboxcryo{Independent operation of the four cold boxes}
\def\dphandlingspecs{Fulfill material handling specification}
\def\dpmaterialbuffer{>1 month}
\def\dpundergroundstorage{>4~\dshorts{crp}}


==> generated/reqdefs-DP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-PDS


\def\dphitrelativetiming{$<\,\SI{100}{ns RMS}$}
\def\dphitsnr{$>\,\num{5}$}
\def\dppdsanalogrange{$>\,\SI{100}{PE/(ch\times 6\nano\second)}$}
\def\dppmtdarkrate{$<\,\SI{100}{kHz}$}


==> generated/reqdefs-SP-APA.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-APA


\def\spapaactivearea{Maximize total active area.}
\def\spapabadchannels{$<$1\%, with a goal of $<$0.5\%}
\def\spapabiasvoltage{The setup, including boards, must hold 150\% of max operating voltage.}
\def\spapaframeplanarity{$<$\SI{5}{mm}}
\def\spapaunitsize{\SI{6.0}{m} tall $\times$ \SI{2.3}{m} wide}
\def\spapawiretension{\SI{6}{N} $\pm$ \SI{1}{N}}


==> generated/reqdefs-SP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CALIB


\def\spdatavolumelaser{$>\SI{184}{TB/yr/10 kt}$}
\def\spdatavolumepns{$>\SI{144}{TB/yr/10 kt}$}
\def\spefieldcalibcoverage{$>\SI{75}{\%}$}
\def\spefieldcalibgranularity{$~30\times 30\times 30~$\SI{}{\centi\metre\cubed}}
\def\spefieldcalibprecision{$\SI{1}{\%}$}
\def\splaserlocationprecision{$~\SI{0.5}{\milli\radian}$}
\def\spneutronsourcecoverage{$>\SI{75}{\%}$}


==> generated/reqdefs-SP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CISC


\def\spcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\speleclifetimeprec{$<\,$1.4\%}
\def\speleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\spinstefield{$<\,\SI{30}{kV/cm}$}
\def\spinstnoise{$<<\,\SI{1000}\,e^- $}
\def\spslowcontrolalarmrate{$<\,$150/day}
\def\spslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\spslowcontrolnumvars{$>\,\num{150000}$}
\def\sptemprepro{$<\,\SI{5}{mK}$}
\def\sptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-SP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-DAQ


\def\spdaqdeadtime{}
\def\spDAQreadout{1.5 TB/s per single phase detector module}
\def\spDAQreadoutwindow{10 $\mu$s < readout window < 100 s}
\def\spDAQthroughput{10 Gb/s average storage throughput; 100 Gb/s peak temporary storage throughput per single phase detector module}
\def\spdatarecord{}
\def\spdataverification{}
\def\sptriggercalibration{}
\def\sptriggerhighenergy{$>$\SI{100}{\MeV}}
\def\sptriggerlowenergy{$>$\SI{10}{\MeV}}


==> generated/reqdefs-SP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-ELEC


\def\spcoldcablesxsec{\SI{6.35}{cm} (2.5")}
\def\spFEMBdatalink{\num{4} at \SI{1.28}{Gbps}}
\def\spgainFEamplifier{$\sim\SI{20}{mV/fC}$}
\def\spnumchannelsFEMB{\num{128}}
\def\spnumFEbaselines{\num{2}}
\def\spnumberFEMBperWIB{\num{4}}
\def\spsyncronizationCE{\SI{50}{ns}}
\def\spWIBdatalink{\SI{10}{Gbps}}


==> generated/reqdefs-SP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-FD


\def\sp{}
\def\spadcnumberofbits{\num{12} bits}
\def\spadcsamplingfreq{$\sim\,\SI{2}{\mega\hertz}$}
\def\spapagaps{$<\,\SI{15}{mm}$ between APAs on same support beam; $<\,\SI{30}{mm}$ between APAs on different support beams}
\def\spapawireangles{\SI{0}{\degree} for collection wires, $\pm\,$\SI{35.7}{\degree} for induction wires}
\def\spapawirepostolerance{$\pm\,\SI{0.5}{mm}$}
\def\spapawirespacing{\SI{4.669}{mm} for U,V; \SI{4.790}{mm} for X,G}
\def\spcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\spcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\spcryomonitordevices{}
\def\spdataratetotape{$<\,\SI{30}{PB/year}$}
\def\spdeadchannels{$<\,\SI{1}{\%}$}
\def\spdpdetmoduptime{$>\,$90\%}
\def\spdpdetuptime{$>\,$98\%}
\def\spfepeaktime{\SI{1}{\micro\second}}
\def\sphvpsripple{$<\,\SI{100}e^-$}
\def\sphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\splarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\splarncontamination{$<\,\SI{25}{ppm}$}
\def\splarpurity{$<$\,\SI{100}{ppt}}
\def\splightyield{$>\,\SI{20}{PE/MeV}$ (avg), $>\,\SI{0.5}{PE/MeV}$ (min)}
\def\splocalefields{$<\,\SI{30}{kV/cm}$}
\def\spmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\spmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\spnonfenoise{$<<\,\SI{1000}\,e^- $}
\def\spradiopurity{less than that from $^{39}$Ar}
\def\spsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\spspsignalsaturation{\num{500000} $e^-$}
\def\spsystemnoise{$<\,\SI{1000}\,e^-$}
\def\sptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-SP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-HV


\def\sphvconnectionredundancy{Two-fold}
\def\sppowersupplystability{$>\,\SI{95}{\%}$ uptime}


==> generated/reqdefs-SP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-INST


\def\spapastoragesd{700 m$^2$}
\def\spcleanroomspecification{ISO 8}
\def\spcleanroomuvfilters{filter $<\SI{400}{nm}$ for $>$ 2 wk exp; $<\SI{520}{nm}$ all else}
\def\splogisticsmaterialhandling{SURF Material Handling Specification}
\def\splogisticsmaterialsbuffer{$>1$ month}
\def\splogisticsshippingcoord{2 wk notice to CMGC}


==> generated/reqdefs-SP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-PDS


\def\spapainstall{$>\,\SI{1}{\milli\meter}$}
\def\spenvhumiditylimit{$<\,\SI{50}{\%}$ RH at \SI{70}{\degree F}}
\def\spenvlightexposure{No exposure to sunlight. All other unfiltered sources: $<\,\num{30}$ minutes integrated across all exposures}
\def\splighttightness{Cryostat light leaks responsible for $<\,\SI{10}{\%}$  of data transferred from PDS to DAQ}
\def\spmechcompatibility{$>\,\SI{1}{\milli\meter}$}
\def\spmechdeflection{$<\,\SI{5}{\milli\meter}$}
\def\sppdscable{$<\,\SI{6}{\milli\meter}$}
\def\sppdscablemate{\SI{0}{\milli\meter} separation mechanically allowed}
\def\sppdscleanroomassbly{Class \num{100000} clean assembly area}
\def\sppdsclearance{$>\,\SI{0.5}{\milli\meter}$}
\def\sppdsdarkrate{$<\,\SI{1}{kHz}$}
\def\sppdsdatarate{$<\,\SI{8}{Gbps}$}
\def\sppdsdynamicrange{$<\,\SI{20}{\%}$}
\def\sppdssignaltonoise{$>\,\num{4}$}
\def\spspatiallocalization{$<\,\SI{2.5}{\meter}$}


==> generated/reqdefs.tex <==
% generated file, do not edit\input{generated/reqdefs-SP-FD}
\input{generated/reqdefs-DP-FD}
\input{generated/reqdefs-SP-APA}
\input{generated/reqdefs-DP-CRP}
\input{generated/reqdefs-SP-HV}
\input{generated/reqdefs-DP-HV}
\input{generated/reqdefs-SP-PDS}
\input{generated/reqdefs-DP-PDS}
\input{generated/reqdefs-SP-DAQ}
\input{generated/reqdefs-DP-DAQ}
\input{generated/reqdefs-SP-CISC}
\input{generated/reqdefs-DP-CISC}
\input{generated/reqdefs-SP-ELEC}
\input{generated/reqdefs-DP-ELEC}
\input{generated/reqdefs-SP-CALIB}
\input{generated/reqdefs-DP-CALIB}
\input{generated/reqdefs-SP-INST}
\input{generated/reqdefs-DP-INST}

